A New Hybrid Automaton Framework with Partial Differential Equation Dynamics

This paper presents the syntax and semantics of a novel type of hybrid automaton (HA) with partial differential equation (PDE) dynamic, partial differential hybrid automata (PDHA). In PDHA, we add a spatial domain $X$ and harness a mathematic conception, partition, to help us formally define the spatial relations. While classically the dynamics of HA are described by ordinary differential equations (ODEs) and differential inclusions, PDHA is capable of describing the behavior of cyber-physical systems (CPS) with continuous dynamics that cannot be modelled using the canonical hybrid systems' framework. For the purposes of analyzing PDHA, we propose another model called the discrete space partial differential hybrid automata (DSPDHA) which handles discrete spatial domains using finite difference methods (FDM) and this simple and intuitive approach reduces the PDHA into HA with ODE systems. We conclude with two illustrative examples in order to exhibit the nature of PDHA and DSPDHA.

==> PDE.tex <==
\section{\textcolor{blue}{Partial Differential Equations (to be deleted)}}\label{sec:pde}

\begin{comment}

%\subsection{General Form}
PDEs are generalizations of ordinary differential equations (ODEs). Instead of involving only one differentiable variable--- time $t$ in the case of ODEs that arise in typical hybrid systems---PDEs utilize derivatives over multiple variables to model state-space dependent evolution with respect to time at every point in a state space. The general form of a PDE is:
\begin{equation}\label{eq:2st}
\begin{split}
0 = & F(\boldsymbol{x}, u(\boldsymbol{x}), \nabla u(\boldsymbol{x}), \Delta u(\boldsymbol{x})) = F(\boldsymbol{x}, u, \nabla u, \Delta u, ), \textrm{ where}\\
\boldsymbol{x} = & (x_1, x_2, \ldots, x_n),\\
\nabla u = & (\pdv{u}{x_1}, \pdv{u}{x_2}, \ldots, \pdv{u}{x_n}),\\
\Delta u = & \pdv[2]{u}{x_1} + \pdv[2]{u}{x_2} + \ldots + \pdv[2]{u}{x_n}
\end{split}
\end{equation}
\noindent
%where $\boldsymbol{x} = (x_1, x_2, \ldots, x_n)$,  $\nabla u = (\pdv{u}{x_1}, \pdv{u}{x_2}, \ldots, \pdv{u}{x_n})$ and $\Delta u = \pdv[2]{u}{x_1} + \pdv[2]{u}{x_2} + \ldots + \pdv[2]{u}{x_n}$ \cite{miersemann2015PDE}.

Usually, as we consider classification of PDEs, it is primarily based on second order equations. The general form of second-order PDE \cite{grigoryan2010PDE} is:
\begin{equation}\label{eq:1st}
\begin{split}
&Au_{xx} + Bu_{xy} + Cu_{yy} + Du_x + Eu_y + Fu = G, \textrm{ where} \\
&u_{xx} = \pdv[2]{u}{x}, u_{xy} = \pdv[2]{u}{x}{y},  u_{yy} = \pdv[2]{u}{y}, u_{x} = \pdv{u}{x}, u_{y} = \pdv{u}{y},\\
&\textrm{and } A, B, C, D, E, F, G \text{ are constants}.
\end{split}
\end{equation}
\noindent 

\end{comment}











%A partial differential equation (PDE) is an equation involving partial derivatives. %This is not so informative so let's break it down.


\begin{comment}

\subsection{Differential Equations}

An ordinary differential equation (ODE) is an equation for a function that depends on one independent variable, involves the independent variable, the function, and derivatives of the function:

\begin{equation}\label{eq:exp1}
\begin{split}
&F(t, u(t), u^{(1)}(t), u^{(2)}(t), u^{(3)}(t),...,u^{(m)}(t)) = 0.\\
\end{split}
\end{equation}

\noindent Equation (\ref{eq:exp1}) is an example of an ODE of degree $m$, where $m$ is the highest order of the derivative in the equation. Solving an equation like this on an interval $t \in [0, T]$ equates to finding a function $t \rightarrow u(t) \in \mathbb{R}$ with the property that $u$ and its derivatives couple in such a way that this equation is true for all values of $t \in [0, T]$. The problem can be expanded to vector-valued functions by replacing the real-valued $u$ by a vector-valued one $u(t) = (u_1(t), u_2(t), . . . , u_N (t))$. In such a case we usually talk about systems of ODEs.

\subsection{Partial Derivative}




When you have function that depends upon several variables, you can differentiate with respect to each variable while holding the other variables constant. This is the basic idea behind \textit{partial derivatives}. As an example, consider a function that depends on two real variables:

\begin{equation}\label{eq:exp}
\begin{split}
&u: \mathbb{R}^n \rightarrow \mathbb{R}.\\
\end{split}
\end{equation}

\noindent For $n = 2$, we sometimes visualize such a function by considering its graph as a surface in $\mathbb{R}^3$ given by the collection of points:


\begin{equation}\label{eq:exp}
\begin{split}
&{(x, y, z) \in \mathbb{R}^3 : z = u(x, y)}.\\
\end{split}
\end{equation}

\end{comment}

%\noindent We can compute the derivative with respect to $x$ while holding $y$ fixed. This yields $u_x$ which can also be expressed as $\partial_xu, \pdv{u}{x}$, and $\pdv{\:}{x}$. Similarly, we can hold $x$ fixed and differentiate with respect to y.

A partial differential equation is an equation for a function that depends on more than one independent variable, involves the independent variables, the function, and the partial derivatives of the function:

\begin{equation}\label{eq:pde_general}
\begin{split}
F(x, y, u(x, y), u_x(x, y), u_y(x, y), u_{xx}(x, y), u_{xy}(x, y), u_{yx}(x, y), u_{yy}(x, y)) = 0.
\end{split}
\end{equation}


Equation (\ref{eq:pde_general}) is an example of a second degree PDE. Solving an equation such as this corresponds to finding a function $(x, y) \rightarrow u(x, y)$ with the property that $u$ and its partial derivatives satisfy equation (\ref{eq:pde_general}). Similarly to the case of ODEs, we can expand equation (\ref{eq:pde_general}) to describe vector valued functions by replacing the real-valued function $u$ with a vector-valued one $\mathbf{u}(t) = (u_1(t), u_2(t), . . . , u_N (t))$. In this framework, we usually talk about a system of PDEs. We can also write (\ref{eq:pde_general}) in its explicit form:

\begin{equation}\label{eq:2st}
\begin{split}
&Au_{xx} + Bu_{xy} + Cu_{yy} + Du_x + Eu_y + Fu + G = 0, \\
&u_{xx} = \pdv[2]{u}{x}, u_{xy} = \pdv[2]{u}{x}{y},  u_{yy} = \pdv[2]{u}{y}, u_{x} = \pdv{u}{x}, u_{y} = \pdv{u}{y},\\
\end{split}
\end{equation}
where $A, B, C, D, E, F, G$ are constants.


As is common in the PDE literature, we write $u_t$ to represent the first order derivative of time, and $u_x$ and $u_{xx}$ to represent the first and second order derivative with respect to space. We refer to $\nabla u$ as the \emph{gradient} of $u$ and $\Delta u$ as the \emph{Laplacian} of $u$. Additionally, some linear, second-order PDEs, can be classified as \textit{parabolic}, \textit{hyperbolic}, or \textit{elliptic}. Table \ref{pdetype} captures the relation between the coefficients in equation (\ref{eq:2st}) and the equation type, providing a guide to specify appropriate initial and boundary conditions and the smoothness of the solutions. %\todo{equation type? undefined term, clarify}.

\begin{table}[t!]
\centering
\begin{tabular}{|l|l|l|}
\hline
Types of PDEs       & Coefficient condition & Examples                                                                               \\ \hline
parabolic equation  & $B^2-AC = 0$          & \begin{tabular}[c]{@{}l@{}}heat equation: \\ $u_t - \alpha \Delta u = f$\end{tabular} \\ \hline
hyperbolic equation & $B^2-AC > 0$          & \begin{tabular}[c]{@{}l@{}}wave equation: \\ $u_{tt} - c^2 u_{xx} = 0$\end{tabular}   \\ \hline
elliptic equation   & $B^2-AC < 0$          & \begin{tabular}[c]{@{}l@{}}Poisson's equation: \\ $\Delta u = f$\end{tabular}         \\ \hline
\end{tabular}%
\caption{The definition of the types of PDEs, their coefficient conditions, and examples.}%\vspace{-1.5em}
\label{pdetype}%
\end{table}

%------------------------------------------------------------------
It is worth noting that in PDE modeling, there is a \emph{domain} of discourse over which the PDE is valid for capturing physical phenomena. From physical intuition, it is necessary to specify boundary conditions in order for the solution to be determined. Table \ref{pdebc} summarizes several useful classes of boundary conditions (BCs). For the \emph{Dirichlet} boundary condition, the value is specified on $\Gamma$. The \emph{Neumann} boundary condition specifies the derivative on $\Gamma$ and the \emph{Robin} boundary condition provides a mixed condition.

\begin{comment}
(1) $u$ is specified (\emph{Dirichlet condition})

(2) the normal derivative $\pdv{u}{n}$ is specified ("\emph{Neumann condition}")

(3) $\pdv{u}{n} + \beta u$ is specified ("\emph{Robin condition}")

\end{comment}

\noindent

\begin{comment}

Consider a heat conduction equation with Dirichlet BC given as:
\begin{equation}\label{eq:exp}
\begin{split}
&\pdv{u}{t} - \Delta u = f(\boldsymbol{x}, t), ~in \: \Omega \\
&u(\boldsymbol{x}) = g(\boldsymbol{x}), ~on \: \Gamma\\
\end{split}
\end{equation}
$\boldsymbol{x} = (x_1, ..., x_n)$, $\Delta$ is the Laplacian defined above in Equation (\ref{eq:2st}), and $\Omega$ is a bounded domain in $d$ dimension Euclidean space $R^n$ with boundary $\Gamma$. The given functions $f(x)$ and $g(x)$ are the data of the problem. 

Instead of Dirichlet boundary condition, one can also consider, for instance, Neumann's boundary condition:

\begin{equation}\label{eq:exp}
\begin{split}
&\pdv{u}{n} = g(\boldsymbol{x}),~on \: \Gamma\\
\end{split}
\end{equation}
%where $\pdv{u}{n}$ denotes the derivative in the direction of the exterior unit normal $n$ to $\Gamma$.
The remaining one is Robin's boundary condition

\begin{equation}\label{eq:exp}
\begin{split}
&\pdv{u}{n} + \beta(\boldsymbol{x})u= g(\boldsymbol{x}),~on \: \Gamma\\
\end{split}
\end{equation}

This will be considered for positive time $t$ and the value of the solution $u$ has to be given at the initial time $t = 0$. In the case of unrestricted space $\mathbb{R}^{n}$ the respective problems are referred to as the pure \emph{initial value problem} or \emph{Cauchy problem} and, in the case of a bounded domain $\Omega$, a mixed \emph{initial-boundary value problem}.

Applied problems often lead to PDEs which are nonlinear. In many cases, it is useful to study linearized versions of these, and the theory of linear equations is therefore relevant also to nonlinear problems.
\end{comment}


%We summarized table \ref{pdebc} for types of boundary conditions below. Frequently the boundary condition serves as a kind of invariant to the hybrid automata.

\begin{table}[t!]
\centering
\begin{tabular}{|l|l|l|}
\hline
Types of BCs & Values on boundary $\Gamma$                                                                                                & Examples                                                                            \\ \hline
Dirichlet     & $u(\boldsymbol{x}) = g(\boldsymbol{x})$                                                                                   & \begin{tabular}[c]{@{}l@{}}fixed temperature is given \\ \\ on  $\Gamma$ for heat equation \end{tabular}           \\ \hline
Neumann       & $\pdv{u}{n} = g(\boldsymbol{x})$                                                                                          & \begin{tabular}[c]{@{}l@{}}wave is reflected on $\Gamma$\\ \\ for wave equation\end{tabular} \\ \hline
Robin         & \begin{tabular}[c]{@{}l@{}}$\pdv{u}{\boldsymbol{x}} + \beta(\boldsymbol{x})u= g(\boldsymbol{x})$\end{tabular} & \begin{tabular}[c]{@{}l@{}}heat exchange is valid  \\ \\ on $\Gamma$ for heat equation \end{tabular}                                                                \\ \hline
\end{tabular}
%
\caption{Types of Boundary Conditions, their values on boundary and examples.}%\vspace{-2.5em}
\label{pdebc}%
\end{table}



